Feature 3DGS: Supercharging 3D Gaussian Splatting to Enable Distilled Feature Fields

3D scene representations have gained immense popularity in recent years. Methods that use Neural Radiance fields are versatile for traditional tasks such as novel view synthesis. In recent times, some work has emerged that aims to extend the functionality of NeRF beyond view synthesis, for semantically aware tasks such as editing and segmentation using 3D feature field distillation from 2D foundation models. However, these methods have two major limitations: (a) they are limited by the rendering speed of NeRF pipelines, and (b) implicitly represented feature fields suffer from continuity artifacts reducing feature quality. Recently, 3D Gaussian Splatting has shown state-of-the-art performance on real-time radiance field rendering. In this work, we go one step further: in addition to radiance field rendering, we enable 3D Gaussian splatting on arbitrary-dimension semantic features via 2D foundation model distillation. This translation is not straightforward: naively incorporating feature fields in the 3DGS framework encounters significant challenges, notably the disparities in spatial resolution and channel consistency between RGB images and feature maps. We propose architectural and training changes to efficiently avert this problem. Our proposed method is general, and our experiments showcase novel view semantic segmentation, language-guided editing and segment anything through learning feature fields from state-of-the-art 2D foundation models such as SAM and CLIP-LSeg. Across experiments, our distillation method is able to provide comparable or better results, while being significantly faster to both train and render. Additionally, to the best of our knowledge, we are the first method to enable point and bounding-box prompting for radiance field manipulation, by leveraging the SAM model. Project website at: https://feature-3dgs.github.io/

==> sec/3_prelim_old.tex <==
\section{Preliminary}
\label{sec:prelim}

\textbf{3D Gaussian Splatting} ~\cite{kerbl20233d} represents 3D scene information with defined properties of gaussians. The method implemented a rather straightforward method in rendering the 2 dimensional scene with 3D gaussians than a heavy parameterized neural network introduced in Neural Radiance Field (NeRF) ~\cite{mildenhall2021nerf}. Each gaussian is a point with spatial locations of the center X  $\in \mathbb{R}^3$, color C $\in \mathbb{R}^3$, scaling factor s $\in \mathbb{R}$, rotation quaternion q $\in \mathbb{R}^4$, and opacity value $\alpha \in \mathbb{R}$.  The rasteriation of each pixel in its' assigned tile adopts a neural point-based method ~\cite{kopanas2021point}:
\begin{equation}
C = \sum_{i \in \mathbb{N}} c_i \alpha_iT_i \quad \text{where} \quad T_i = \prod_{j=1}^{i-1} (1 - \alpha_j)
\end{equation}
where $\mathbb{N}$ is the sorted gaussians of one pixel, $c_i$ is the color of each gaussian, and $\alpha_i$ is the opacity value of the gaussian. $T_i$ is defined as the product of opacity values of previous gaussian overlapping the same pixel. The optimization process calculates the L1 loss and SSIM loss of the RGB image, and updates the optimization pairs {$X$, $C$, $s$, $q$, $\alpha$} directly. Moreover, each gaussian is splitted or pruned if the view-space gradient is greater than the threshold.

\textbf{Foundation models} in AI refer to large-scale models that are pre-trained on vast and diverse datasets, enabling them to develop a wide range of capabilities. These models are called "foundation" because they provide a base layer of knowledge and skills that can be adapted or fine-tuned for a variety of specific tasks and applications. The \textit{Segment Anything Model (SAM)} ~\cite{kirillov2023segment} represents a groundbreaking advancement in the realm of foundation models, specifically tailored for the field of computer vision. As a state-of-the-art model, SAM is trained on an unprecedented scale, leveraging the SA-1B dataset that comprises over 11 million images and 1.1 billion masks. Unique in its capability, SAM excels at both promptable and promptless zero-shot segmentation, allowing it to accurately segment images it has never encountered before, without the need for specific task training or human guidance. Natural language is another widely used modality in foundation models. The Contrastive Language–Image Pretraining (CLIP) model~\cite{radford2021learning}  seamlessly integrates the realms of natural language processing and computer vision, learning to correlate text with corresponding images. This enables the model to grasp visual concepts through the lens of natural language, enhancing its versatility across various visual tasks. Building on this advancement, LSeg ~\cite{li2022languagedriven} introduces a language-driven approach to zero-shot semantic segmentation. Utilizing the image feature encoder with the DPT architecture~\cite{ranftl2021vision} and text encoders from CLIP, LSeg extends text-image associations to a pixel-level granularity. This approach allows for more precise segmentation of unseen images by mapping semantically related labels to analogous areas in the images, aligning them within a nuanced, high-dimensional embedding space. Furthermore, large models like ALIGM ~\cite{jia2021scaling}, CoCa ~\cite{yu2022coca}, and DINO ~\cite{caron2021dino} have shown great generality to leverage their capabilities for more downstream tasks. 

Our proposed method is general and compatible with any 2D foundation model, distilling the semantic features into a 3D feature field using 3D Gaussian splatting. In our experiments, we employ SAM and LSeg, facilitating both promptable and language-driven computer vision tasks in a 3D context.
